ReaRev: Adaptive Reasoning for Question Answering over Knowledge Graphs

Knowledge Graph Question Answering (KGQA) involves retrieving entities as answers from a Knowledge Graph (KG) using natural language queries. The challenge is to learn to reason over question-relevant KG facts that traverse KG entities and lead to the question answers. To facilitate reasoning, the question is decoded into instructions, which are dense question representations used to guide the KG traversals. However, if the derived instructions do not exactly match the underlying KG information, they may lead to reasoning under irrelevant context. Our method, termed ReaRev, introduces a new way to KGQA reasoning with respect to both instruction decoding and execution. To improve instruction decoding, we perform reasoning in an adaptive manner, where KG-aware information is used to iteratively update the initial instructions. To improve instruction execution, we emulate breadth-first search (BFS) with graph neural networks (GNNs). The BFS strategy treats the instructions as a set and allows our method to decide on their execution order on the fly. Experimental results on three KGQA benchmarks demonstrate the ReaRev's effectiveness compared with previous state-of-the-art, especially when the KG is incomplete or when we tackle complex questions. Our code is publicly available at https://github.com/cmavro/ReaRev_KGQA.

==> tables/meta_app.tex <==
\begin{table}[tb]
	\centering
	\caption{Performance comparison of different methods for KGQA (Hits@1 or F1 scores in \%). Bold fonts denote the best methods. }
	\label{tab:res}%
	%\begin{small}
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{@{}lcc@{}}
			%\cline{3-7}
			\toprule
			% &\multicolumn{2}{c}{Webqsp}&\multicolumn{2}{c}{MetaQA-1}&\multicolumn{2}{c}{MetaQA-2}&\multicolumn{2}{c}{MetaQA-3}&\multicolumn{2}{c}{CWQ}\\
			 & \textbf{MetaQA-2} & \textbf{MetaQA-3} \\
			% Models&Hits&F1&Hits&F1&Hits&F1&Hits&F1&Hits&F1\\
			\midrule
			GNN-based Methods & & \\
			Answer Coverage & 100 & 99.0 \\
			Answer Recall & 98.3 & 92.3 \\
			GraftNet~\cite{sun2018open} & 94.8 & 77.7 \\
			PullNet~\cite{sun2019pullnet} & 99.9 & 91.4 \\
			NSM~\cite{he2021improving}	& 99.9 & 98.9  \\
			NSM-distill~\cite{he2021improving} & 99.9 & 98.9 \\
			\method & 99.9 & 98.9 \\
			\midrule
			Non GNN-based Methods & & \\
			Answer Coverage & 100 & 100 \\
			Answer Recall & 100 & 100 \\
			KV-Mem~\cite{miller2016key} & 82.7 & 48.9 \\
			ReifKB~\cite{cohen2020scalable} & 95.4 & 79.7\\
			EmQL~\cite{sun2020faithful} & 98.6  & 99.1  \\
			SQALER~\cite{atzeni2021sqaler} & 99.9  & 99.9 \\
			TransferNet~\cite{shi2021transfernet} & 100  & 100 \\
			\bottomrule
		\end{tabular}%
		}
	%\end{small}
\end{table}%


%%%
% model dfs: webqsp: 72.1/67.3


% & Webqsp& CWQ &  MetaQA-2 & MetaQA-3 \\
% 			Models & H@1 / F1 &  H@1 / F1 & H@1 & H@1 \\
% 			% Models&Hits&F1&Hits&F1&Hits&F1&Hits&F1&Hits&F1\\
% 			\midrule
% 			KV-Mem&	46.7 / 38.6& 21.1 / \ \ \ -- &  82.7& 48.9\\
% 			KAReader & 67.2 / 57.3  & -- &  -- & -- \\
% 			GraftNet & 66.7 / 62.4  & 32.8 / \ \ \ -- &  94.8& 77.7 \\
% 			PullNet & 68.1 / \; -- \; & 45.9 / \ \ \ -- &  \textbf{99.9}& 91.4 \\
% 			SRN & -- &  -- &  95.1& 75.2\\
% 			EmbedKGQA &	66.6 / \; -- \; & -- &  98.8 & 94.8\\
% 			NSM	&	68.7 / 62.8 & 47.6 / 42.4 &  \textbf{99.9}& \textbf{98.9}\\
% 			NSM-distill & \textbf{74.3} / 67.4 & 48.8 / 44.0  & \textbf{99.9}& \textbf{98.9}\\
% 			\hline
% 			\textbf{BFS} & &  &  &  \\
% 			\; \methodg & 69.5 / 64.6 & 48.3 / 45.6 &  99.8 & 97.5  \\
% 			\; \method & 73.3 / 68.9 & \textbf{50.4} / \textbf{46.3} &  \textbf{99.9} & \textbf{98.9} \\
% 			\textbf{DFS} & &  &  &  \\
% 			\; \methodg & 72.6 / 68.4 &  &  \textbf{99.9} & \textbf{98.9}  \\
% 			\; \method & 74.0 / \textbf{69.7} & 49.3 / 46.6 &  \textbf{99.9} & \textbf{98.9} \\
